Turnaround radius in $f(R)$ model

We investigate the turnaround radius in the spherical collapse model, both in General Relativity and in modified gravity, in particular $f(R)$ scenarios. The phases of spherical collapse are marked by the density contrast in the instant of turnaround $\delta_t$, and by the linear density contrast in the moment of collapse, $\delta_c$. We find that the effective mass of the extra scalar degree of freedom which arises in modified gravity models has an impact on $\delta_t$ of up to $\sim10\%$, and that $\delta_c$ can increase by $\sim1.0\%$. We also compute the turnaround radius, $R_t$, which in modified gravity models can increase by up to $\sim 6\%$ at $z \simeq 0$.

==> bibliografia.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage

\addcontentsline{toc}{chapter}{Referências}

% Referências =====================================================================%
\begin{thebibliography}{12cm}

\bibitem{Riess} Riess, A. G., et al., 2004, ApJ, 607, 655

\bibitem{permutter} S. Perlmutter, et al., 2004, Astrophysics, 607, 655

\bibitem{WessZumino1} Wess, J. and Zumino, B., {\it Nuclear Physics}, {\bf B70}, 39 (1974).

\bibitem{Ryder} Ryder, L. H. {\it Quantum Field Theory}. Cambridge University Press, 1996
(Second Edition).


\bibitem{Grad} Gradshteyn, I. S, Ryzhik, I. M. {\it Table of Integrals, Series and Products: 
Corrected and Enlarged Edition}. Academic Press, Inc. San Diego, 1980.

\end{thebibliography}

%==================================================================================%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

